STORNS: Stochastic Radio Access Network Slicing

Recently released 5G networks empower the novel Network Slicing concept. %which enables novel business models; Network slicing introduces new business models such as allowing telecom providers to lease a virtualized slice of their infrastructure to tenants such as industry verticals, e.g. automotive, e-health, factories, etc. However, this new paradigm poses a major challenge when applied to Radio Access Networks (RAN): how to achieve revenue maximization while meeting the diverse service level agreements (SLAs) requested by the infrastructure tenants? In this paper, we propose a new analytical framework, based on stochastic geometry theory, to model realistic RANs that leverage the business opportunities offered by network slicing. We mathematically prove the benefits of slicing radio access networks as compared to non-sliced infrastructures. Based on this, we design a new admission control functional block, STORNS, which takes decisions considering per slice SLA guaranteed average experienced throughput. A radio resource allocation strategy is introduced to optimally allocate transmit power and bandwidth (i.e., a slice of radio access resources) to the users of each infrastructure tenant. Numerical results are illustrated to validate our proposed solution in terms of potential spectral efficiency, and compare it against a non-slicing benchmark.

==> design.tex <==
\section{Problem Design}
\label{s:design}

We envisage a network with multiple access points, such as LTE eNB, femto-cells, mm-waves access points. Tenant $i\in\mathcal{I}$ is willing to pay for using the radio access network (RAN) facilities given certain SLAs, e.g., average throughput. Users $u\in\mathcal{U}_i$ are associated with a particular tenant $i$ with user density $\lambda_i$.

\subsection{Toy scenario}

Let us consider a toy scenario for shedding the light on our system and correctly identify the pillars of our problem. We assume a homogeneous network deployment, e.g., LTE eNBs with a given bandwidth $BW$ and maximum transmission power $P_{\text{TX}}$. Given the tenant SLAs in terms of average throughput, i.e., $\text{Th}_i = \alpha_i \text{Th}$ where Th is the maximum throughput the network can provide, and considering only two tenants $i=\{1,2\}$ and the same user density $\lambda_1 = \lambda_2$, we can formulate the following optimization problem:

\vspace{2mm}\noindent \textbf{Problem}~\texttt{Bi-Sharing}:
\begin{equation*}
\label{pr:bi-sharing}
\begin{array}{ll}
\text{minimize}  & \mathbbm{1}\\
\text{subject to } & B_1\left(1\! -\! e^{-(\frac{P_1}{B_1})^{2/ \beta}}\right)\!\! \geq \alpha_1 BW\!\left( 1\!-\!e^{-(\frac{P_{\text{TX}}}{BW})^{2/ \beta}} \right);\\
				   & B_2\left(1\! -\! e^{-(\frac{P_2}{B_2})^{2/ \beta}}\right)\!\! \geq \alpha_2 BW\!\left( 1\!-\!e^{-(\frac{P_{\text{TX}}}{BW})^{2/ \beta}} \right);\\
				   & B_1 + B_2 \leq BW;\\
				   & P_1 + P_2 \leq P_{\text{TX}};\\
                   & B_1, B_2, P_1, P_2 \in \mathbb{R}_{+};
\end{array}
\end{equation*}
where on the right side the total achievable throughput $\text{Th} = BW\left( 1-e^{(\frac{P_{\text{TX}}}{BW})^{2/ \beta}} \right)$ is derived. When $P_i = B_i$, we can derive the following set of inequalities:
\begin{equation}
\begin{array}{ll}
B_1 C & \geq \alpha_1 K;\\
B_2 C & \geq \alpha_2 K;\\
B_1 + B_2 & \leq B;
\end{array}
\end{equation}
where $C = 1-e^{(-2/ \beta)}$ and $K = BW\left( 1-e^{-(\frac{P_{\text{TX}}}{BW})^{2/ \beta}} \right)$. By fixing $B_1$ with the least feasible value $B_1=\frac{\alpha_1K}{C}$, we can derive the admissibility region of $B_2$, i.e., $\frac{\alpha_2K}{C} \leq B_2 \leq BW-\frac{\alpha_1K}{C}$.

Generally speaking, Problem~\texttt{Bi-Sharing} provides the optimal set of values $B_i \in\mathcal{B}$ and $P_i\in\mathcal{P}$ given the tenants SLAs.

\begin{proposition}
\label{prop:convexity}
Given the set of convex constraints, Problem~\texttt{Bi-Sharing} is optimally solved through gradient descent algorithm.
\end{proposition}

Proposition~\ref{prop:convexity} relies on the convexity property of the multivariable function $g(x,y) = g(B_1,P_1) = B_1\left(1 - e^{-(\frac{P_1}{B_1})} \right)$. We first check the Hessian condition for convexity, as follows: 

\[
H_{g(x,y)}
=
\begin{bmatrix}
    \frac{\partial^{2} g(x,y)}{\partial x^2 } & \frac{\partial^{2} g(x,y)}{\partial x \partial y } \\
    \frac{\partial^{2} g(x,y)}{\partial y \partial x} & \frac{\partial^{2} g(x,y)}{\partial y^2 }
\end{bmatrix}
=
\begin{bmatrix}
    -\frac{e^{-x/y}}{y} & \frac{xe^{-x/y}}{y^2} \\
    \frac{xe^{-x/y}}{y^2} & -\frac{x^2e^{-x/y}}{y^3}
\end{bmatrix},
\]
where $\det(H_{g(x,y)}) = 0$. Therefore, we need to check the following condition:
\begin{equation}
g(tx_1 + (1-t)x_2,ty_1 + (1-t)y_2) \leq tg(x_1,y_1) + (1-t)g(x_2,y_2).
\end{equation}
Analytically, it holds that 
\begin{equation}
\begin{array}{ll}
g(tx_1 + (1-t)x_2,ty_1 + (1-t)y_2) & =\\
(ty_1 +(1-t)y_2) (1-e^{-\frac{tx_1 + (1-t)x_2}{ty_1 + (1-t)y_2}}) & \leq \\
(ty_1 +(1-t)y_2) (\frac{ty_1}{ty_1+(1-t)y_2}(1-e^{-\frac{x_1}{y_1}}) \\+\frac{(1-t)y_2}{ty_1+(1-t)y_2}(1-e^{-\frac{x_2}{y_2}})) & = \\
ty_1(1-e^{-\frac{x_1}{y_1}})+(1-t)y_2(1-e^{-\frac{x_2}{y_2}}) & = \\
tg(x_1,y_1)+(1-t)g(x_2,y_2). & 
\end{array}
\end{equation}
The second inequality holds because of the convexity of $f(x)=1-e^{-x}$.

\subsection{Heterogeneous Tenant Distributions}

\newcounter{mytempeqncnt}
\begin{figure*}[b]
\hrulefill
\normalsize
\setcounter{mytempeqncnt}{\value{equation}}
\begin{equation}
\begin{array}{l}
\lambda_{\text{BS}} \hat\Omega\left(\frac{\lambda_i}{\lambda_{\text{BS}}}\right)B_i\log(1+\gamma_I)\frac{1}{1+\hat\Omega\left(\frac{\lambda_i}{\lambda_{\text{BS}}}\right)\Gamma(\gamma_I)} \left[ 1-\exp\left(-\pi\lambda_{\text{BS}}\left(\frac{P_i}{K B_i}\frac{1}{N_0 \gamma_I} \right)^{2/\beta} \left(1+\hat\Omega\left(\frac{\lambda_i}{\lambda_{\text{BS}}}\right)\Gamma(\gamma_I) \right) \right) \right] \geq \alpha_i \text{Th}\\
\text{where}\quad \hat\Omega(\frac{\lambda_i}{\lambda_{\text{BS}}}) = 1 - \left( 1+ \frac{1}{3.5} \frac{\lambda_i }{\lambda_{\text{BS}}} \right)^{-3.5} \geq 0; \\
\text{and}\quad \Gamma(\gamma_I) = \;_2\!F_1 \left(-\frac{2}{\beta},1,1-\frac{2}{\beta},-\gamma_I\right)-1 \geq 0.
\end{array}
\label{eq:diff_lambda}
\end{equation}
\setcounter{equation}{\value{mytempeqncnt}} 
%\hrulefill
\end{figure*}

\vspace{2mm}\noindent \textbf{Problem}~\texttt{MultiTenant-Optimizer}:
\begin{equation*}
\label{pr:mt_optimizer}
\begin{array}{ll}
\text{minimize}  & \mathbbm{1}\\
\text{subject to } & \text{Eq.~\eqref{eq:diff_lambda}}, \quad \forall i\in I\\
				   & \sum_i B_i \leq BW;\\
				   & \sum_i P_i \leq P_{\text{TX}};\\
                   & \forall B_i, P_i \in \mathbb{R}_{+};
\end{array}
\end{equation*}


\begin{equation}
\min_{B_1,P_1,B_2,P_2} \max_{\lambda_1,\lambda_2} \lambda_1(\text{Eq.~\eqref{eq:diff_lambda}}) + \lambda_2(\text{Eq.~\eqref{eq:diff_lambda}})
\end{equation}

We can now an iterative subgradient update to optimize the Lagrange multipliers, which regulate the separate solutions of both subproblems:
\begin{align}
 &\mu_{\tau, p, i}^{(k+1)} = \left [ \mu_{\tau,p,i}^{(k)} + \alpha_k \Big (   z_{\tau,p,i} - C_{\tau,p,i}^M x_{\tau,p,i}      \Big ) \right ]^+\label{eq:update1}\\
 &\nu_{\tau, p, i}^{(k+1)} = \left [ \nu_{\tau,p,i}^{(k)} + \alpha_k \Big (   K_{\tau,i}x_{\tau,p,i} -  z_{\tau,p,i}      \Big ) \right ]^+\label{eq:update2}
\end{align}
